On Small Pair Decompositions for Point Sets

$\newcommand{\Re}{\mathbb{R}}$We study the minWSPD problem of computing the minimum-size well-separated pairs decomposition of a set of points, and show constant approximation algorithms in low-dimensional Euclidean space and doubling metrics. This problem is computationally hard already $\Re^2$, and is also hard to approximate. We also introduce a new pair decomposition, removing the requirement that the diameters of the parts should be small. Surprisingly, we show that in a general metric space, one can compute such a decomposition of size $O( \tfrac{n}{\varepsilon}\log n)$, which is dramatically smaller than the quadratic bound for WSPDs. In $\Re^d$, the bound improves to $O( d \tfrac{n}{\varepsilon}\log \tfrac{1}{\varepsilon } )$.

==> figs/tbl_cubes.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $12$ &   $15$ &   $19$ &   $15$ &   $12$ &   $12$ &   $12$ &   $12$
         \\
        \hline
          $20$ &  $190$ &   $31$ &   $38$ &   $46$ &   $38$ &   $31$ &   $31$ &   $31$ &   $31$
         \\
        \hline
          $30$ &  $435$ &   $52$ &   $64$ &   $75$ &   $62$ &   $50$ &   $50$ &   $50$ &   $50$
         \\
        \hline
          $40$ &  $780$ &   $72$ &   $90$ &  $106$ &   $86$ &   $70$ &   $70$ &   $70$ &   $70$
         \\
        \hline
          $50$ & $1,225$ &   $94$ &  $120$ &  $137$ &  $112$ &   $89$ &   $89$ &   $89$ &   $89$
         \\
        \hline
          $60$ & $1,770$ &  $114$ &  $145$ &  $169$ &  $138$ &  $109$ &  $109$ &  $109$ &  $109$
         \\
        \hline
          $70$ & $2,415$ &  $135$ &  $171$ &  $199$ &  $168$ &  $129$ &  $129$ &  $131$ &  $130$
         \\
        \hline
          $80$ & $3,160$ &  $163$ &  $203$ &  $231$ &  $190$ &  $149$ &  $149$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $180$ &  $226$ &  $263$ &  $215$ &  $170$ &  $169$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $204$ &  $259$ &  $297$ &  $242$ &  $190$ &  $188$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $247$ &  $316$ &  $362$ &  $295$ &  $230$ &  $228$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $293$ &  $368$ &  $429$ &  $345$ &  $274$ &  $268$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $343$ &  $427$ &  $496$ &  $399$ &  $315$ &  $309$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $383$ &  $482$ &  $562$ &  $450$ &  $362$ &  $349$ & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $427$ &  $541$ &  $629$ &  $505$ &  $406$ &  $389$ & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $543$ &  $686$ &  $799$ &  $640$ &  $519$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $654$ &  $822$ &  $968$ &  $771$ &  $628$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $774$ &  $962$ & $1,138$ &  $904$ &  $739$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $888$ & $1,112$ & $1,309$ & $1,045$ &  $848$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_log.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $14$ &   $18$ &   $26$ &   $15$ &   $14$ &   $14$ &   $14$ &   $14$
         \\
        \hline
          $20$ &  $190$ &   $37$ &   $44$ &   $68$ &   $42$ &   $33$ &   $33$ &   $34$ &   $34$
         \\
        \hline
          $30$ &  $435$ &   $59$ &   $71$ &  $108$ &   $67$ &   $53$ &   $53$ &   $54$ &   $54$
         \\
        \hline
          $40$ &  $780$ &   $82$ &  $100$ &  $154$ &   $95$ &   $73$ &   $73$ &   $74$ &   $74$
         \\
        \hline
          $50$ & $1,225$ &   $99$ &  $127$ &  $194$ &  $122$ &   $93$ &   $93$ &   $94$ &   $94$
         \\
        \hline
          $60$ & $1,770$ &  $126$ &  $156$ &  $238$ &  $150$ &  $114$ &  $114$ &  $115$ &  $115$
         \\
        \hline
          $70$ & $2,415$ &  $138$ &  $185$ &  $280$ &  $178$ &  $134$ &  $134$ &  $138$ &  $135$
         \\
        \hline
          $80$ & $3,160$ &  $174$ &  $211$ &  $326$ &  $207$ &  $155$ &  $155$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $195$ &  $241$ &  $369$ &  $237$ &  $176$ &  $175$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $213$ &  $269$ &  $411$ &  $261$ &  $197$ &  $195$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $259$ &  $326$ &  $499$ &  $320$ &  $240$ &  $235$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $310$ &  $384$ &  $587$ &  $376$ &  $285$ &  $276$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $355$ &  $437$ &  $672$ &  $431$ &  $326$ &  $317$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $411$ &  $497$ &  $760$ &  $490$ &  $375$ &  $358$ & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $452$ &  $558$ &  $850$ &  $549$ &  $449$ & -- & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $564$ &  $693$ & $1,066$ &  $692$ &  $569$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $686$ &  $841$ & $1,287$ &  $836$ &  $686$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $819$ &  $989$ & $1,506$ &  $981$ &  $803$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $925$ & $1,125$ & $1,722$ & $1,123$ &  $923$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_log_sq.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $15$ &   $17$ &   $28$ &   $16$ &   $14$ &   $14$ &   $14$ &   $14$
         \\
        \hline
          $20$ &  $190$ &   $38$ &   $43$ &   $68$ &   $40$ &   $33$ &   $33$ &   $33$ &   $33$
         \\
        \hline
          $30$ &  $435$ &   $60$ &   $71$ &  $112$ &   $68$ &   $53$ &   $53$ &   $54$ &   $54$
         \\
        \hline
          $40$ &  $780$ &   $85$ &   $99$ &  $153$ &   $96$ &   $73$ &   $73$ &   $74$ &   $74$
         \\
        \hline
          $50$ & $1,225$ &  $102$ &  $127$ &  $195$ &  $122$ &   $93$ &   $93$ &   $94$ &   $94$
         \\
        \hline
          $60$ & $1,770$ &  $125$ &  $155$ &  $239$ &  $151$ &  $114$ &  $114$ &  $118$ &  $114$
         \\
        \hline
          $70$ & $2,415$ &  $148$ &  $181$ &  $282$ &  $178$ &  $135$ &  $135$ &  $137$ &  $135$
         \\
        \hline
          $80$ & $3,160$ &  $173$ &  $207$ &  $326$ &  $206$ &  $155$ &  $155$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $203$ &  $240$ &  $368$ &  $232$ &  $176$ &  $175$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $221$ &  $270$ &  $411$ &  $263$ &  $197$ &  $195$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $267$ &  $323$ &  $499$ &  $320$ &  $240$ &  $235$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $310$ &  $381$ &  $587$ &  $376$ &  $283$ &  $276$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $358$ &  $441$ &  $674$ &  $437$ &  $327$ &  $317$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $409$ &  $500$ &  $761$ &  $491$ &  $391$ & -- & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $449$ &  $553$ &  $848$ &  $548$ &  $437$ & -- & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $569$ &  $691$ & $1,069$ &  $693$ &  $549$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $696$ &  $841$ & $1,287$ &  $837$ &  $663$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $801$ &  $982$ & $1,505$ &  $980$ &  $776$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $925$ & $1,119$ & $1,725$ & $1,128$ &  $893$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_normal.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $12$ &   $12$ &   $13$ &   $12$ &   $12$ &   $12$ &   $12$ &   $12$
         \\
        \hline
          $20$ &  $190$ &   $29$ &   $30$ &   $34$ &   $32$ &   $29$ &   $29$ &   $29$ &   $29$
         \\
        \hline
          $30$ &  $435$ &   $50$ &   $61$ &   $67$ &   $57$ &   $46$ &   $46$ &   $47$ &   $47$
         \\
        \hline
          $40$ &  $780$ &   $65$ &   $80$ &   $83$ &   $71$ &   $61$ &   $61$ &   $62$ &   $62$
         \\
        \hline
          $50$ & $1,225$ &   $82$ &   $91$ &  $100$ &   $89$ &   $75$ &   $75$ &   $75$ &   $75$
         \\
        \hline
          $60$ & $1,770$ &  $106$ &  $114$ &  $132$ &  $114$ &   $93$ &   $93$ &   $94$ &   $94$
         \\
        \hline
          $70$ & $2,415$ &  $122$ &  $133$ &  $156$ &  $133$ &  $109$ &  $109$ &  $110$ &  $110$
         \\
        \hline
          $80$ & $3,160$ &  $142$ &  $154$ &  $186$ &  $152$ &  $127$ &  $127$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $152$ &  $176$ &  $207$ &  $179$ &  $143$ &  $143$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $174$ &  $205$ &  $219$ &  $190$ &  $158$ &  $158$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $216$ &  $249$ &  $292$ &  $243$ &  $192$ &  $192$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $257$ &  $286$ &  $324$ &  $284$ &  $228$ &  $227$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $284$ &  $318$ &  $373$ &  $317$ &  $259$ &  $258$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $319$ &  $382$ &  $419$ &  $357$ &  $290$ &  $290$ & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $366$ &  $427$ &  $461$ &  $395$ &  $323$ &  $322$ & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $445$ &  $518$ &  $581$ &  $499$ &  $428$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $554$ &  $623$ &  $743$ &  $626$ &  $529$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $651$ &  $749$ &  $832$ &  $713$ &  $618$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $757$ &  $883$ &  $980$ &  $847$ &  $712$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_squares.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $13$ &   $16$ &   $20$ &   $16$ &   $13$ &   $13$ &   $13$ &   $13$
         \\
        \hline
          $20$ &  $190$ &   $34$ &   $41$ &   $49$ &   $38$ &   $32$ &   $32$ &   $32$ &   $32$
         \\
        \hline
          $30$ &  $435$ &   $54$ &   $69$ &   $80$ &   $62$ &   $52$ &   $52$ &   $52$ &   $52$
         \\
        \hline
          $40$ &  $780$ &   $78$ &   $96$ &  $110$ &   $91$ &   $71$ &   $71$ &   $71$ &   $71$
         \\
        \hline
          $50$ & $1,225$ &   $97$ &  $122$ &  $142$ &  $115$ &   $91$ &   $91$ &   $92$ &   $92$
         \\
        \hline
          $60$ & $1,770$ &  $120$ &  $150$ &  $175$ &  $143$ &  $111$ &  $111$ &  $112$ &  $112$
         \\
        \hline
          $70$ & $2,415$ &  $142$ &  $176$ &  $208$ &  $169$ &  $131$ &  $131$ &  $133$ &  $132$
         \\
        \hline
          $80$ & $3,160$ &  $164$ &  $208$ &  $241$ &  $190$ &  $152$ &  $152$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $186$ &  $235$ &  $274$ &  $218$ &  $172$ &  $172$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $211$ &  $258$ &  $307$ &  $244$ &  $193$ &  $192$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $254$ &  $320$ &  $374$ &  $299$ &  $236$ &  $232$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $298$ &  $376$ &  $441$ &  $350$ &  $280$ &  $272$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $347$ &  $436$ &  $509$ &  $404$ &  $320$ &  $312$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $392$ &  $490$ &  $577$ &  $465$ &  $365$ &  $353$ & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $432$ &  $542$ &  $645$ &  $518$ &  $417$ & -- & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $548$ &  $688$ &  $815$ &  $646$ &  $523$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $664$ &  $832$ &  $986$ &  $787$ &  $629$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $783$ &  $975$ & $1,157$ &  $921$ &  $737$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $893$ & $1,112$ & $1,328$ & $1,060$ &  $848$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_uniform.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $12$ &   $15$ &   $14$ &   $12$ &   $12$ &   $12$ &   $12$ &   $12$
         \\
        \hline
          $20$ &  $190$ &   $30$ &   $36$ &   $38$ &   $31$ &   $29$ &   $29$ &   $29$ &   $29$
         \\
        \hline
          $30$ &  $435$ &   $49$ &   $55$ &   $63$ &   $51$ &   $45$ &   $45$ &   $47$ &   $47$
         \\
        \hline
          $40$ &  $780$ &   $69$ &   $82$ &   $86$ &   $72$ &   $63$ &   $63$ &   $65$ &   $65$
         \\
        \hline
          $50$ & $1,225$ &   $87$ &  $111$ &  $112$ &   $91$ &   $81$ &   $81$ &   $84$ &   $82$
         \\
        \hline
          $60$ & $1,770$ &  $108$ &  $122$ &  $139$ &  $113$ &   $98$ &   $98$ &  $105$ &  $100$
         \\
        \hline
          $70$ & $2,415$ &  $126$ &  $143$ &  $162$ &  $132$ &  $116$ &  $115$ &  $122$ &  $118$
         \\
        \hline
          $80$ & $3,160$ &  $146$ &  $177$ &  $189$ &  $156$ &  $134$ &  $132$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $167$ &  $207$ &  $216$ &  $177$ &  $152$ &  $149$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $188$ &  $236$ &  $239$ &  $196$ &  $170$ &  $166$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $228$ &  $259$ &  $293$ &  $240$ &  $208$ &  $201$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $265$ &  $302$ &  $344$ &  $283$ &  $242$ &  $236$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $308$ &  $368$ &  $395$ &  $325$ &  $285$ &  $271$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $345$ &  $430$ &  $450$ &  $371$ &  $335$ & -- & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $387$ &  $489$ &  $501$ &  $414$ &  $374$ & -- & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $501$ &  $546$ &  $630$ &  $520$ &  $473$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $591$ &  $692$ &  $763$ &  $630$ &  $573$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $696$ &  $837$ &  $893$ &  $740$ &  $672$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $797$ &  $998$ & $1,023$ &  $848$ &  $771$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}


==> figs/tbl_urand.tex <==
\centering
\begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{{ |r|r|r|r|r|r|r|r|r|r| }}
        \hline
        n & N & Greedy & WSPD & Aprx3 & Aprx3C & IP & IP$_{LB}$ & IP DJ & IP DJ$_{LB}$ \\
         \hline
        \hline
          $10$ &   $45$ &   $10$ &   $10$ &   $14$ &   $11$ &   $10$ &   $10$ &   $10$ &   $10$
         \\
        \hline
          $20$ &  $190$ &   $27$ &   $30$ &   $37$ &   $31$ &   $27$ &   $27$ &   $27$ &   $27$
         \\
        \hline
          $30$ &  $435$ &   $50$ &   $62$ &   $65$ &   $52$ &   $45$ &   $45$ &   $45$ &   $45$
         \\
        \hline
          $40$ &  $780$ &   $63$ &   $74$ &   $85$ &   $70$ &   $59$ &   $59$ &   $60$ &   $60$
         \\
        \hline
          $50$ & $1,225$ &   $76$ &   $89$ &   $99$ &   $88$ &   $72$ &   $72$ &   $72$ &   $72$
         \\
        \hline
          $60$ & $1,770$ &   $97$ &  $120$ &  $128$ &  $109$ &   $91$ &   $91$ &   $92$ &   $92$
         \\
        \hline
          $70$ & $2,415$ &  $119$ &  $140$ &  $157$ &  $129$ &  $108$ &  $108$ &  $109$ &  $109$
         \\
        \hline
          $80$ & $3,160$ &  $146$ &  $163$ &  $184$ &  $159$ &  $130$ &  $130$ & -- & --
         \\
        \hline
          $90$ & $4,005$ &  $163$ &  $184$ &  $210$ &  $170$ &  $142$ &  $142$ & -- & --
         \\
        \hline
         $100$ & $4,950$ &  $171$ &  $203$ &  $227$ &  $191$ &  $158$ &  $158$ & -- & --
         \\
        \hline
         $120$ & $7,140$ &  $203$ &  $235$ &  $266$ &  $221$ &  $183$ &  $183$ & -- & --
         \\
        \hline
         $140$ & $9,730$ &  $247$ &  $285$ &  $319$ &  $273$ &  $223$ &  $223$ & -- & --
         \\
        \hline
         $160$ & $12,720$ &  $277$ &  $318$ &  $373$ &  $317$ &  $256$ &  $256$ & -- & --
         \\
        \hline
         $180$ & $16,110$ &  $315$ &  $378$ &  $398$ &  $345$ &  $282$ &  $282$ & -- & --
         \\
        \hline
         $200$ & $19,900$ &  $359$ &  $416$ &  $470$ &  $398$ &  $324$ &  $322$ & -- & --
         \\
        \hline
         $250$ & $31,125$ &  $438$ &  $515$ &  $565$ &  $476$ &  $424$ & -- & -- & --
         \\
        \hline
         $300$ & $44,850$ &  $548$ &  $631$ &  $693$ &  $590$ &  $527$ & -- & -- & --
         \\
        \hline
         $350$ & $61,075$ &  $655$ &  $748$ &  $840$ &  $724$ &  $625$ & -- & -- & --
         \\
        \hline
         $400$ & $79,800$ &  $737$ &  $823$ &  $949$ &  $814$ &  $696$ & -- & -- & --
         \\
        \hline
    \end{tabular}
\end{adjustbox}

